Towards a Logic for Reasoning About LF Specifications

We describe the development of a logic for reasoning about specifications in the Edinburgh Logical Framework (LF). In this logic, typing judgments in LF serve as atomic formulas, and quantification is permitted over contexts and terms that might appear in them. Further, contexts, which constitute type assignments to uniquely named variables that are modeled using the technical device of nominal constants, can be characterized via an inductive description of their structure. We present a semantics for such formulas and then consider the task of proving them. Towards this end, we restrict the collection of formulas we consider so as to ensure that they have normal forms upon which proof rules may be based. We then specifically discuss a proof rule that provides the basis for case analysis over LF typing judgments; this rule is the most complex and innovative one in the collection. We illustrate the proof system through an example. Finally, we discuss ongoing work and we relate our project to existing systems that have a similar goal.

==> soundness.tex <==
\label{sec:soundness}
\section{Soundness and Consistency}

In this section we consider an approach to showing the soundness of our proof
rules relative to the semantics given to formulas based on derivability in LF.
%
Using this result we will also be able to show consistency of the overall system.
%
We propose the following statement for soundness.

\noindent{\bf Soundness:} If the sequent
$\seq{\mathcal{C}}{\Psi}{\Delta}{F}$ is derivable then given a ground
LF context satisfying the schema annotation for each context given
in $\mathcal{C}$ and ground terms for each eigenvariable in $\Psi$,
if the formulas given in $\Delta$ are all valid in LF then the formula
$F$ is valid in LF. 

The general approach to soundness we will take is to show the property 
inductively over the derivations in our proof system.
%
We will consider the definition of each proof rule and show that it is
itself sound with respect to the notion of derivability in LF given
by the semantics we have defined.
%
We consider in more detail how this argument might work out for
the case analysis rule we describe in Section~\ref{sec:rules}.

In the case analysis rule we can classify the cases into three
categories based on what declaration was used in the derivation under
consideration.
%
The first is the use of an object level constant from the signature.
%
Second we have those that come from using an object level variable
from either the specified part of the context or an existing block in
the unspecified part of he context.
%
Finally we may have used an object level variable from an unspecified
block in the unspecified part of the context.
%
Given the derivation rules for LF these three categories cover all the
possible ways to derive a judgment of the form
$\{\lfprove{\Sigma}{G}{M:A}\}$, so what we must argue is that the way
we are generating the cases covers all valid possibilities in LF for
each category.

In the first two situations described above we do consider each
possible entry and so can ensure that any case which would result in a
valid LF derivation will be covered by something in our set.
%
For the last case, while we consider every possible block
structure in every possible position within the context, we do prune
out some cases through the raising that is done.
%
However, these cases are not in fact possible in LF; any eigenvariable
which we do not raise over the newly introduced names will have a
first occurrence in a type to the left of where these names appear in
the context.
%
This means that any instantiate of this eigenvariable which makes use
of these names results in a context which is not valid in LF by
introducing a dependency on something which comes later in the
context.

Once soundness is established the existence of well-formed formulas
which are not derivable (and thus not true in LF) demonstrates the
consistency of the overall system.
%
As an example consider the property that for any
term and type in the simply typed lambda calculus there is a
derivation that that particular term has that particular type.
%
the following formula which uses the encoding
of typing in the simply typed lambda calculus from
Figure~\ref{fig:stlc} would capture such a property.
%
\[
\forall E\forall T.
\{\lfprove{\Sigma}{\cdot}{E:tm}\}\supset
\{\lfprove{\Sigma}{\cdot}{T:ty}\}\supset
\exists D.\{\lfprove{\Sigma}{\cdot}{D:of~E~T}\}
\]
%
This is well-formed in the sense we have defined in
Section~\ref{sec:rules}, but will not be derivable for obvious
reasons.
